Large Language Models and Causal Inference in Collaboration: A Survey

Causal inference has shown potential in enhancing the predictive accuracy, fairness, robustness, and explainability of Natural Language Processing (NLP) models by capturing causal relationships among variables. The emergence of generative Large Language Models (LLMs) has significantly impacted various NLP domains, particularly through their advanced reasoning capabilities. This survey focuses on evaluating and improving LLMs from a causal view in the following areas: understanding and improving the LLMs' reasoning capacity, addressing fairness and safety issues in LLMs, complementing LLMs with explanations, and handling multimodality. Meanwhile, LLMs' strong reasoning capacities can in turn contribute to the field of causal inference by aiding causal relationship discovery and causal effect estimations. This review explores the interplay between causal inference frameworks and LLMs from both perspectives, emphasizing their collective potential to further the development of more advanced and equitable artificial intelligence systems.

==> ARR/ARR_Sections/LLM_for_Causal/assumptions.tex <==
\subsection{Fundamental Assumptions in Estimating Treatment Effect }
\label{subsec:assumptions}

% Xiaoyu

In existing causal inference literature, several assumptions are adopted to estimate the treatment effect. Here we discuss the three most commonly used assumptions and then show how the development of large language models could help relax or challenge these fundamental assumptions.


\begin{assumption}[\textbf{Stable Unit Treatment Value Assumption} ]
The potential outcomes for any unit do not vary with the treatment assigned to other units, and, for each unit, there are no different forms or versions of each treatment level, which leads to different potential outcomes.
\end{assumption}

This assumption emphasizes the independence of each unit when estimating the treatment effect that the units do not interact with each other. From a statistical perspective, it is equivalent to assuming each treatment assignment subject is iid. 


\begin{assumption}[\textbf{Unconfoundedness} ]
\label{ass:causal-2}
Given the observable background variable, X, treatment assignment T is independent of
the potential outcomes.
\end{assumption}

The \cref{ass:causal-2} states that if the background variable $X$ is the same for two patients, then (1) the treatment assignment should be the same. (2) the potential outcome should also be the same. In other words, these two patients are treated as identical units, thus can be used to estimate the treatment effect if they are assigned different treatments in the static dataset, as the treatment assignment is treated as random. 

\begin{assumption}[\textbf{Positivity} ]
\label{ass:causal-3}
For any value of X, treatment assignment is not deterministic. i.e.,

\begin{equation}
    P(T=t|X=x) > 0, \forall t, x
\end{equation}
\end{assumption}

This assumption tries to guarantee that the treatment effect can be estimated and that we can always find a comparable sample. In the binary case, if the task is to estimate the performance of a specific treatment $T=1$, we would need to compare the potential outcome of patients receiving the treatment against those who are not treated, requiring dataset points in both cases.








